A Regression-Based Share Market Prediction Model for Bangladesh

Share market is one of the most important sectors of economic development of a country. Everyday almost all companies issue their shares and investors buy and sell shares of these companies. Generally investors want to buy shares of the companies whose market liquidity is comparatively greater. Market liquidity depends on the average price of a share. In this paper, a thorough linear regression analysis has been performed on the stock market data of Dhaka Stock Exchange. Later, the linear model has been compared with random forest based on different metrics showing better results for random forest model. However, the amount of individual significance of different factors on the variability of stock price has been identified and explained. This paper also shows that the time series data is not capable of generating a predictive linear model for analysis.

==> tab_pca.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!th]
\centering
\caption{Loading Vectors of First and Second Principle Components (Values with absolute loadings $\geq$ 0.5 are bolded)}
\label{pca}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Variables} & \textbf{PC1}    & \textbf{PC2}    & \textbf{PC3}    & \textbf{PC4}    & \textbf{PC5}   \\ \hline
ol                 & -0.066          & 0.348           & 0.275           & 0.333           & 0.427          \\ \hline
lr                 & \textbf{0.677}  & 0.232           & 0.157           & -0.265          & -0.073         \\ \hline
isb                & \textbf{0.65}   & -0.268          & 0.294           & 0.125           & -0.072         \\ \hline
hs                 & -0.044          & \textbf{-0.785} & 0.362           & 0.141           & 0.22           \\ \hline
ihm                & 0.457           & 0.237           & 0.447           & -0.392          & -0.148         \\ \hline
hhm                & -0.036          & \textbf{0.601}  & -0.091          & 0.282           & -0.076         \\ \hline
cck                & 0.215           & 0               & 0.485           & 0               & 0.229          \\ \hline
dmk                & 0.167           & -0.049          & -0.355          & 0.222           & -0.26          \\ \hline
or                 & \textbf{-0.528} & 0.448           & -0.05           & 0.153           & -0.104         \\ \hline
ph                 & 0.038           & \textbf{0.56}   & 0.139           & -0.097          & 0.018          \\ \hline
mlr                & \textbf{0.805}  & 0.268           & 0.111           & -0.065          & 0.165          \\ \hline
ll                 & -0.281          & -0.207          & \textbf{0.632}  & 0.035           & -0.051         \\ \hline
rl                 & -0.347          & -0.348          & -0.173          & 0.055           & -0.114         \\ \hline
rf                 & 0               & \textbf{-0.754} & -0.032          & 0.014           & 0.207          \\ \hline
hmd                & 0.162           & 0.339           & -0.071          & \textbf{0.705}  & -0.13          \\ \hline
el                 & -0.302          & 0.061           & -0.478          & \textbf{-0.574} & 0.108          \\ \hline
lrs                & \textbf{0.558}  & 0.440           & 0.006           & -0.223          & 0.138          \\ \hline
lrg                & 0.36            & \textbf{0.623}  & -0.217          & -0.059          & 0.088          \\ \hline
oln                & -0.032          & 0.288           & 0.31            & 0.287           & \textbf{0.579} \\ \hline
isa                & \textbf{-0.562} & 0.480           & 0.09            & -0.08           & 0.258          \\ \hline
sra                & \textbf{0.718}  & -0.266          & 0.106           & 0.147           & -0.248         \\ \hline
fa                 & -0.336          & -0.164          & -0.075          & 0.126           & 0.382          \\ \hline
hsw                & 0               & -0.247          & 0.192           & -0.43           & 0.291          \\ \hline
htw                & \textbf{-0.573} & 0.113           & 0.323           & -0.097          & -0.321         \\ \hline
hrw                & 0.394           & -0.198          & \textbf{-0.549} & -0.108          & 0.427          \\ \hline
hws                & 0.162           & -0.092          & -0.406          & 0.171           & 0.323          \\ \hline
prp                & \textbf{0.761}  & -0.294          & -0.199          & 0.215           & -0.053         \\ \hline
\end{tabular}%
}
\end{table}


==> table-smmary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[!ht]
\centering
\caption{Coefficients   of   Linear   Regression   Analysis(***p <0.0001, *p <0.05)}
\label{datasummary}
\begin{tabular}{|p{2.2cm}|p{3cm}|p{2.2cm}|p{2.2cm} | p{2.2cm}|}
\hline
\textbf{Predictors} & \textbf{Estimate}  & \textbf{Std. Error} & \textbf{t- Value} & \textbf{Pr(>|t|)}  \\ \hline
(Intercept) &  -1691.838 & 167.744 &  -10.086 &  1.55$e^{-14}$ ***  \\  \cline{1-5} 
Term &  42.113 & 7.348 &  5.731 &  3.44$e^{-07}$ *** \\  \cline{1-5} 
ROE  & 342,091   & 902.390 & 0.379 &  0.706 \\ \cline{1-5}  
CR &  -32.597 & 15.769 & -2.067 &  0.043 \\ \cline{1-5}*  
TATO & 2367.872  & 824.498 & 8.515 &  3.02$e^{-05}$ *** \\ \cline{1-5}  
DTA & 2536.810  & 308.046 & 8.235 &  1.95$e^{-11}$ ***\\ \cline{1-5}  
Panel & 213.175 & 31.151 & 6.843 & 4.63$e^{-09}$ ***  \\ \hline 


\end{tabular}
\end{table*}


==> table_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\begin{table*}[!ht]
\centering
\caption{Predictor Name and Data Source}
\label{data_data}
\begin{tabular}{|p{2.5cm}|p{4.7cm}|p{2.2cm}|p{2.2cm} |}
\hline
\textbf{Predictor Name} & \textbf{F-Statistics}  & \textbf{$R^2$} & \textbf{RSE} \\ \hline
COMID &  1424 & 0.0103 &  283.1 \\  \cline{1-4} 
LOWPRC*  & $2.242\times10^8$   & 0.9994 & 6.983  \\ \cline{1-4}  
HIPRC* &  $1.382\times10^8$ & 0.999 & 8.893  \\ \cline{1-4}  
AVGPRC* &  $1.362\times10^9$  & 0.9999 & 2.834  \\ \cline{1-4}  
WTAVGPRC* & $1.23\times10^9$  & 0.9999 & 2.982 \\ \cline{1-4}  
TRDNO & 40.41 &0.0003 & 284.6 \\ \cline{1-4} 
TRDVOL & 1563  & 0.0114 & 283 \\ \cline{1-4} 
ISSUEDSHARE & 2452  & 0.0178 & 282.1  \\ \cline{1-4} 
TURNOVER & 359  & 0.0027 & 284.2  \\ \hline

\end{tabular}
\end{table*}

